Beyond Transfer Learning: Co-finetuning for Action Localisation

Transfer learning is the predominant paradigm for training deep networks on small target datasets. Models are typically pretrained on large ``upstream'' datasets for classification, as such labels are easy to collect, and then finetuned on ``downstream'' tasks such as action localisation, which are smaller due to their finer-grained annotations. In this paper, we question this approach, and propose co-finetuning -- simultaneously training a single model on multiple ``upstream'' and ``downstream'' tasks. We demonstrate that co-finetuning outperforms traditional transfer learning when using the same total amount of data, and also show how we can easily extend our approach to multiple ``upstream'' datasets to further improve performance. In particular, co-finetuning significantly improves the performance on rare classes in our downstream task, as it has a regularising effect, and enables the network to learn feature representations that transfer between different datasets. Finally, we observe how co-finetuning with public, video classification datasets, we are able to achieve state-of-the-art results for spatio-temporal action localisation on the challenging AVA and AVA-Kinetics datasets, outperforming recent works which develop intricate models.

==> tables/cofinetuning_copretraining_rebuttal.tex <==
\begin{table}[t]
	\centering
	\caption{
		Comparison of traditional finetuning, co-pretraining and co-finetuning.
		``Total Iter.'' denotes the total training iterations of all stages.
		We follow the same settings as Table 2 of the paper.
	}
	\vspace{-0.75\baselineskip}
	\scalebox{0.79}{
		\begin{tabular}{cccccc}
			\toprule
			Pretrain & Finetune & AVA & K400 & MiT & Total Iter.\\
			\midrule
			\multicolumn{6}{l}{\textit{Traditional transfer}} \\
			K400 & MiT & -- & -- & 37.2 & 178.8k \\ %
			MiT & K400 & -- & 76.3  & -- & 178.8k \\ %
			MiT$\to$K400 & AVA & 25.1 & -- & -- & 211.8k \\ %
			\midrule
			\multicolumn{6}{l}{\textit{Co-pretraining}} \\
			MiT + K400 & -- &  -- & \textbf{76.7} & 38.5  & 178.8k \\
			MiT + K400 & AVA & 25.5  & -- &  -- & 211.8k \\  %
			\midrule
			\multicolumn{6}{l}{\textit{Co-finetuning}} \\
			-- & MiT + K400 + AVA & \textbf{26.3} & \textbf{76.7} & \textbf{38.9} & 211.8k\\ %
			\bottomrule
		\end{tabular}
	}
	\vspace{-1.5\baselineskip}
	\label{tab:cofinetune_updated}
\end{table}
